On the seed population of solar energetic particles in the inner heliosphere

Particles measured in large gradual solar energetic particle (SEP) events are believed to be predominantly accelerated at shocks driven by coronal mass ejections (CMEs). Ion charge state and composition analyses suggest that the origin of the seed particle population for the mechanisms of particle acceleration at CME-driven shocks is not the bulk solar wind thermal material, but rather a suprathermal population present in the solar wind. This suprathermal population could result from remnant material accelerated in prior solar flares and/or preceding CME-driven shocks. In this work, we examine the distribution of this suprathermal particle population in the inner heliosphere by combining a magnetohydrodynamic (MHD) simulation of the solar wind and a Monte-Carlo simulation of particle acceleration and transport. Assuming that the seed particles are uniformly distributed near the Sun by solar flares of various magnitudes, we study the longitudinal distribution of the seed population at multiple heliocentric distances. We consider a non-uniform background solar wind, consisting of fast and slow streams that lead to compression and rarefaction regions within the solar wind. Our simulations show that the seed population at a particular location (e.g., 1 au) is strongly modulated by the underlying solar wind configuration. Corotating interaction regions (CIRs) and merged interactions regions (MIRs) can strongly alter the energy spectra of the seed particle populations. In addition, cross-field diffusion plays an important role in mitigating strong variations of the seed population in both space and energy.

==> Arxiv On the seed population of solar energetic particles in the inner heliosphere (JGR)/abbrev.tex <==
\usepackage{xspace}
\newcommand{\aj}{AJ\xspace}
\newcommand{\apj}{ApJ}
\newcommand{\apjl}{ApJ\xspace}
\newcommand{\apjlett}{ApJ\xspace}
\newcommand{\apjs}{ApJS\xspace}
\newcommand{\apjsupp}{ApJS\xspace}
\newcommand{\aap}{A\&A}
\newcommand{\astap}{A\&A\xspace}
\newcommand{\araa}{ARA\&A\xspace}
\newcommand{\aapr}{A\&A Rev.\xspace}
\newcommand{\aaps}{A\&AS\xspace}
\newcommand{\mnras}{MNRAS\xspace}
\newcommand{\pasp}{PASP\xspace}
\newcommand{\apss}{Ap\&SS\xspace}
\newcommand{\pasj}{PASJ\xspace}
\newcommand{\nat}{Nature\xspace}
\newcommand{\sci}{Science\xspace}
\newcommand{\skytel}{S\&T\xspace}
\newcommand{\memras}{MmRAS\xspace}
\newcommand{\qjras}{QJRAS\xspace}
\newcommand{\jrasc}{JRASC\xspace}
\newcommand{\baas}{BAAS\xspace}
\newcommand{\iauc}{IAU Circ.\xspace}
\newcommand{\iaucirc}{IAU Circ.\xspace}
\newcommand{\aplett}{Astrophys. Lett.\xspace}
\newcommand{\apspr}{Astrophys. Space Phys. Res.\xspace}
\newcommand{\bain}{Bull. Astron. Inst. Netherlands\xspace}
\newcommand{\fcp}{Fund. Cosmic Phys.\xspace}
\newcommand{\aipconf}{AIP Conf. Proc.\xspace}
\newcommand{\aspconf}{ASP Conf. Ser.\xspace}
\newcommand{\asslconf}{Ap\&SSL Conf. Ser.\xspace}
\newcommand{\procspie}{Proc. SPIE\xspace}
\newcommand{\maps}{MAPS\xspace}
\newcommand{\planss}{Planet. Space Sci.\xspace}
\newcommand{\ssr}{Space Sci. Rev.}
\newcommand{\ao}{Appl. Opt.\xspace}
\newcommand{\applopt}{Appl. Opt.\xspace}
\newcommand{\solphys}{Sol. Phys.}
\newcommand{\pra}{Phys. Rev. A\xspace}
\newcommand{\prb}{Phys. Rev. B\xspace}
\newcommand{\prc}{Phys. Rev. C\xspace}
\newcommand{\prd}{Phys. Rev. D\xspace}
\newcommand{\pre}{Phys. Rev. E\xspace}
\newcommand{\prl}{Phys. Rev. Lett.\xspace}
\newcommand{\rmp}{Rev. Mod. Phys.\xspace}
\newcommand{\grl}{Geophys. Res. Lett.}
\newcommand{\jgr}{J. Geophys. Res.\xspace}
\newcommand{\adv}{Adv. Space Res.\xspace}
\newcommand{\icrc}{ICRC}
\newcommand{\jswsc}{J. Space Weather Space Clim.}
\newcommand{\jcp}{	J. Chem. Phys.}
\newcommand{\jpp}{	J. Plasma Phys.}
